Solving Energy-Independent Density for CT Metal Artifact Reduction via Neural Representation

X-ray CT often suffers from shadowing and streaking artifacts in the presence of metallic materials, which severely degrade imaging quality. Physically, the linear attenuation coefficients (LACs) of metals vary significantly with X-ray energy, causing a nonlinear beam hardening effect (BHE) in CT measurements. Reconstructing CT images from metal-corrupted measurements consequently becomes a challenging nonlinear inverse problem. Existing state-of-the-art (SOTA) metal artifact reduction (MAR) algorithms rely on supervised learning with numerous paired CT samples. While promising, these supervised methods often assume that the unknown LACs are energy-independent, ignoring the energy-induced BHE, which results in limited generalization. Moreover, the requirement for large datasets also limits their applications in real-world scenarios. In this work, we propose Density neural representation (Diner), a novel unsupervised MAR method. Our key innovation lies in formulating MAR as an energy-independent density reconstruction problem that strictly adheres to the photon-tissue absorption physical model. This model is inherently nonlinear and complex, making it a rarely considered approach in inverse imaging problems. By introducing the water-equivalent tissues approximation and a new polychromatic model to characterize the nonlinear CT acquisition process, we directly learn the neural representation of the density map from raw measurements without using external training data. This energy-independent density reconstruction framework fundamentally resolves the nonlinear BHE, enabling superior MAR performance across a wide range of scanning scenarios. Extensive experiments on both simulated and real-world datasets demonstrate the superiority of our unsupervised Diner over popular supervised methods in terms of MAR performance and robustness.

==> section/author_bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/wuqing2.jpg}}]{Qing Wu}(Graduate Student Member, IEEE) received the B.Eng. degree in Communications Engineering from China University of Geosciences, Wuhan, China, in 2020. He is currently pursuing the Ph.D. degree in ShanghaiTech University, Shanghai, China. His current research interests include medical image reconstruction and implicit neural representation.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/xuguo.jpg}}]{Xu Guo} received the B.S. degree in Animal Science from Northwest AF University, Shaanxi, China, in 2021. She is currently pursuing the M.S. degree in ShanghaiTech University, Shanghai, China. Her current research interests include macrophage-stem cell interaction and fracture healing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/chenlixuan.jpg}}]{Lixuan Chen} received the B.Eng. degree in Computer Science and Technology from ShanghaiTech University, Shanghai, China, in 2021. She is currently pursuing the M.S. degree in ShanghaiTech University, Shanghai, China. Her current research interests include medical imaging, deep learning, and image processing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/dongminghe.jpg}}]{DongMing He} currently works at the Department of Oral and Craniomaxillofacial Surgery, Shanghai Ninth People’s Hospital as an attending surgeon, and carrying out researches at Shanghai Key Laboratory of Stomatology, Shanghai, China. He received his Ph.D. degree from West China School of Stomatology, SiChuan University (SCU) in 2018. His research focuses on biomaterials, regenerative medicine, and digital surgical technology.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/hongjiangwei.jpg}}]{Hongjiang Wei} received the B.Eng. degree from the Department of Electronic Information Engineering, Harbin Institute of Technology, Harbin, China, in 2008, the M.Sc. degree from the Department of Electronic Information Engineering, Harbin Institute of Technology, in 2010, and the Ph.D. degree from the Institute National des Sciences Appliquees de Lyon, Lyon, France, in 2014. He is currently with the School of Biomedical Engineering of Shanghai Jiao Tong University, Shanghai, China, specializing in fast MRI, deep learning, and quantitative susceptibility mapping.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/xudongwang.jpg}}]{Xudong Wang} M.D., Chief Physician. He is currently the vice president of the Ninth People's Hospital affiliated with Shanghai Jiaotong University School of Medicine, the chairman of the Oral and Maxillofacial Trauma and Orthognathic Specialized Committee of the Chinese Stomatological Association, and the vice president of the Council of Precision and Digital Medicine Branch of the Chinese Society of Plastic and Aesthetic Surgery. He is mainly engaged in the research of the precision and minimally invasive treatments of orthognathic surgery and distraction osteogenesis for the difficult congenital or acquired dental and maxillofacial malformations. He has published 139 papers, more than 40 authorized patents.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/skevinzhou.jpg}}]{S. Kevin Zhou}(Fellow, IEEE) received his PhD degree from University of Maryland, College Park. Currently he is a distinguished professor and founding executive dean of School of Biomedical Engineering, University of Science and Technology of China (USTC) and an adjunct professor at Institute of Computing Technology, Chinese Academy of Sciences and Chinese University of Hong Kong (CUHK), Shenzhen. Prior to this, he was a principal expert and a senior R\&D director at Siemens Healthcare Research. Dr. Zhou has published 250+ book chapters and peer-reviewed journal and conference papers, registered 140+ granted patents, written three research monographs, and edited three books. The two recent books he led the edition are entitled "Deep Learning for Medical Image Analysis, SK Zhou, H Greenspan, DG Shen (Eds.)" and "Handbook of Medical Image Computing and Computer Assisted Intervention, SK Zhou, D Rueckert, G Fichtinger (Eds.)". He has won multiple awards including R\&D 100 Award (Oscar of Invention), Siemens Inventor of the Year, UMD ECE Distinguished Alumni Award, BMEF Editor of the Year, Finalist Paper for MICCAI Young Scientist Award (twice). He has been a program co-chair for MICCAI 2020, an associate editor for IEEE \textsc{Transactions on Medical Imaging}, IEEE \textsc{Transactions on Pattern Analysis and Machine Intelligence}, and \textit{Medical Image Analysis,} and an area chair for AAAI, CVPR, ICCV, MICCAI, and NeurIPS. He has been elected as a treasurer and board member of the MICCAI Society, an advisory board member of MONAI (Medical Open Network for AI), and a fellow of AIMBE, IAMBE, IEEE, MICCAI, and NAI (National Academy of Inventors).
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/zhangyifeng.jpg}}]{Yifeng Zhang} received his bachelor’s degree in Clinical Medicine in Shanxi Medical University in 2006. In 2007, he studied nanomaterials’ biosafety in College of Engineering, Peking University, and received his master's degree in Biomedical Engineering in 2010. Then, he did the researches about the mechanism of Mg’s osteogenesis effect in Prince of Wales Hospital, The Chinese University of Hong Kong in 2011. In 2015, Dr. Zhang obtained his PhD degree. From 2015 to 2019, Dr Zhang explored several biomedical directions based on Mg ions’ bioactivities, such as bone fracture repair, osteoarthritis, tendon repair, et al. in School of Medicine, Nanjing University. In 2019, Dr. Zhang joined in School of Life Science and Technology, ShanghaiTech University, and established research group of Sports Medicine.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/jingyiyu.jpg}}]{Jingyi Yu}(Fellow, IEEE) received BS from Caltech in 2000 and the Ph.D. degree from MIT in 2005. He is currently the Vice Provost at ShanghaiTech University. Before joining ShanghaiTech, he was a full professor in the Department of Computer and Information Sciences at University of Delaware. His research interests span a range of topics in computer vision and computer graphics, especially on computational photography and nonconventional optics and camera designs. He is a recipient of the NSF CAREER Award and the AFOSR YIP Award, and has served as an area chair of many international conferences including CVPR, ICCV, ECCV, IJCAI and NeurIPS. He was a program chair of CVPR 2021 and will be a program chair of ICCV 2025. He has been an associate editor of IEEE \textsc{Transactions on Pattern Analysis and Machine Intelligence}. He is currently an associate editor of IEEE \textsc{Transactions on Image Processing}, and \textit{Elsevier Computer Vision and Image Understanding}. He is a fellow of IEEE. 
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/zhangyuyao.jpg}}]{Yuyao Zhang}(Member, IEEE) received the B.Eng. degree from the Department of Electronic Information Engineering, Harbin Engineering University, Harbin, China, in 2007 and the M.Sc. degree from the Department of Electronic Information Engineering, Harbin Institute of Technology, Harbin, in 2010, and the Ph.D. degree from the Institut National des Sciences Appliquees de Lyon, Lyon, France, in 2014. She currently works in School of Information Science and Technology of Shanghaitech University, specializing in medical image processing.
\end{IEEEbiography}

==> tables/table_discrete_energy_spectrum.tex <==
\begin{table}[t]
    \centering
    \caption{Quantitative results of our Diner with different spectrum priors $\eta$ on the DeepLesion dataset~\cite{deeplesion}.}
    \label{table:discrete_energy_spectrum}
    \begin{tabular}{lcc}
    \toprule
     \textbf{Discrete Spectrum}    & PSNR & SSIM \\ \midrule
     $N=1$    & 22.45$\pm$4.64 & 0.8050$\pm$0.1529\\
     $N=5$    & 35.64$\pm$1.48 & 0.9799$\pm$0.0063 \\
     $N=10$   & 37.66$\pm$1.30 & 0.9848$\pm$0.0029 \\
     $N=40$   & 39.01$\pm$1.35 & \textbf{0.9845$\pm$0.0029} \\
     $N=81$   & \underline{39.18$\pm$1.44} & \textbf{0.9845$\pm$0.0029} \\
     $N=101$   & \textbf{39.19$\pm$1.44} & \underline{0.9844$\pm$0.0029} \\
     \toprule
    \end{tabular}
\end{table}

==> tables/table_dl.tex <==
\begin{table*}[t]
\centering
\caption{Quantitative results of compared methods for three types of metals on the DeepLesion~\cite{deeplesion} simulation dataset. The best and second performances are respectively highlighted in \textbf{bold} and \underline{underline}.}
\label{table_dl}
% \resizebox{0.95\textwidth}{!}{
\begin{tabular}{clcccccc} 
\toprule
\multirow{4}{*}{\textbf{Category}}     & \multirow{4}{*}{\textbf{Method}} & \multicolumn{6}{c}{\textbf{Types of Metallic Implants}} \\
\cmidrule{3-8}
                              &                         & \multicolumn{2}{c}{\textsc{Titanium}}   & \multicolumn{2}{c}{\textsc{Chromium}} & \multicolumn{2}{c}{\textsc{304 Stainless Steel}}\\ \cmidrule{3-8}
&                         & PSNR           & SSIM            & PSNR           & SSIM             & PSNR           & SSIM\\ 
\midrule
\multirow{2}{*}{\texttt{Model-based}}  & FBP~\cite{fbp}                     & 30.61$\pm$2.71               & 0.7829$\pm$0.0804                & 26.67$\pm$2.89               & 0.6465$\pm$0.1052  & 25.01$\pm$2.95    & 0.5888$\pm$0.1098\\
& LI~\cite{kalender1987li}                     & 32.07$\pm$2.61              & 0.8650$\pm$0.0518                & 32.07$\pm$2.61               & 0.8650$\pm$0.0518 & 32.07$\pm$2.61 & 0.8650$\pm$0.0518  \\
\midrule
\multirow{3}{*}{\texttt{Supervised}}   & CNN-MAR~\cite{cnnmar}                & 35.05$\pm$2.31               & 0.9385$\pm$0.0218                & 34.71$\pm$2.38              & 0.9322$\pm$0.0257       & 34.50$\pm$2.44        & 0.9277$\pm$0.0289 \\
                              & DICDNet~\cite{wang2021dicdnet}                & 37.93$\pm$1.89               & 0.9710$\pm$0.0094                & 37.18$\pm$2.21               & 0.9654$\pm$0.0128    & 36.74$\pm$2.47 & 0.9623$\pm$0.0148 \\
                              & ACDNet~\cite{wang2022acdnet}                 & \underline{38.43$\pm$1.91}               & 0.9701$\pm$0.0112               & \underline{37.46$\pm$2.25}              & 0.9586$\pm$0.0171   & \underline{36.90$\pm$2.50} & 0.9524$\pm$0.0200           \\ 
\midrule
\multirow{3}{*}{\texttt{Unsupervised}} & ADN~\cite{adn2019_tmi}            & 33.49$\pm$2.30               & 0.9481$\pm$0.0153                & 33.65$\pm$2.44               & 0.9492$\pm$0.0159   & 33.58$\pm$2.43  & 0.9487$\pm$0.0159\\
& Polyner~\cite{wu2023unsupervised}                    & 37.26$\pm$1.96             & \underline{0.9766$\pm$0.0056}                 & 37.14$\pm$2.00               & \underline{0.9762$\pm$0.0053}  & 37.05$\pm$2.06 & \underline{0.9759$\pm$0.0061}\\
& Diner (Ours)                    & \textbf{39.15$\pm$1.85}               & \textbf{0.9844$\pm$0.0037}               & \textbf{38.71$\pm$1.81}               & \textbf{0.9821$\pm$0.0046}   & \textbf{38.52$\pm$1.80}
     & \textbf{0.9811$\pm$0.0049}\\
\bottomrule
\end{tabular}
\end{table*}

==> tables/table_polychromatic_image.tex <==
\begin{table}[ht]
    \centering
    \caption{Quantitative results of polychromatic CT images reconstructed by our Diner and Polynner~\cite{wu2023unsupervised} for three types of metals on the DeepLesion dataset~\cite{deeplesion}.}
    \label{table:polychromatic_images}
    \begin{tabular}{llcc}
    \toprule
     \textbf{Method} & \textbf{Types of Metals}  & PSNR & SSIM \\ \midrule
     \multirow{3}{*}{Polyner~\cite{wu2023unsupervised}}    & \textsc{Titanium} &29.75$\pm$5.16 & 0.9349$\pm$0.0738\\
      &\textsc{Chromium}  & 29.71$\pm$5.14 & 0.9336$\pm$0.0736 \\
     &\textsc{Stainless Steel}  & 29.54$\pm$5.00 & 0.9320$\pm$0.0732 \\ \midrule
     \multirow{3}{*}{Diner (Ours)}    & \textsc{Titanium} &\textbf{37.31$\pm$2.36} & \textbf{0.9820$\pm$0.0052}\\
      &\textsc{Chromium}  & \textbf{37.05$\pm$2.28} & \textbf{0.9800$\pm$0.0056} \\
     &\textsc{Stainless Steel}  & \textbf{36.92$\pm$2.24} & \textbf{0.9790$\pm$0.0059} \\
     \toprule
    \end{tabular}
\end{table}

==> tables/table_xcom.tex <==
\begin{table}[t]
\centering
\caption{Quantitative results of compared methods on the XCOM~\cite{deeplesion} simulation dataset. The best and second performances are respectively highlighted in \textbf{bold} and \underline{underline}.}
\label{table_xcom}
\begin{tabular}{clcc} 
\toprule
\textbf{Category}     & \textbf{Method} & PSNR           & SSIM \\
\midrule
\multirow{2}{*}{\texttt{Model-based}}  & FBP~\cite{fbp}                     & 30.90$\pm$4.70               & 0.6988$\pm$0.1622\\
& LI~\cite{kalender1987li}                     & 33.15$\pm$0.53            & 0.8813$\pm$0.0262\\
\midrule
\multirow{3}{*}{\texttt{Supervised}}   & CNN-MAR~\cite{cnnmar}                & \underline{38.04$\pm$0.81}               & 0.9464$\pm$0.0130\\
                              & DICDNet~\cite{wang2021dicdnet}                & 34.39$\pm$1.71               & 0.9481$\pm$0.0100\\
                              & ACDNet~\cite{wang2022acdnet}                 & 34.18$\pm$2.68              & 0.9456$\pm$0.0113\\ 
\midrule
\multirow{3}{*}{\texttt{Unsupervised}} & ADN~\cite{adn2019_tmi}            & 30.61$\pm$1.20               & 0.9152$\pm$0.0296      \\
& Polyner~\cite{wu2023unsupervised}                    & 37.63$\pm$0.35             & \textbf{0.9684$\pm$0.0141}\\
& Diner (Ours)                    & \textbf{38.90$\pm$0.48}               & \underline{0.9670$\pm$0.0075}\\
\bottomrule
\end{tabular}
\end{table}
